TIFu: Tri-directional Implicit Function for High-Fidelity 3D Character Reconstruction

Recent advances in implicit function-based approaches have shown promising results in 3D human reconstruction from a single RGB image. However, these methods are not sufficient to extend to more general cases, often generating dragged or disconnected body parts, particularly for animated characters. We argue that these limitations stem from the use of the existing point-level 3D shape representation, which lacks holistic 3D context understanding. Voxel-based reconstruction methods are more suitable for capturing the entire 3D space at once, however, these methods are not practical for high-resolution reconstructions due to their excessive memory usage. To address these challenges, we introduce Tri-directional Implicit Function (TIFu), which is a vector-level representation that increases global 3D consistencies while significantly reducing memory usage compared to voxel representations. We also introduce a new algorithm in 3D reconstruction at an arbitrary resolution by aggregating vectors along three orthogonal axes, resolving inherent problems with regressing fixed dimension of vectors. Our approach achieves state-of-the-art performances in both our self-curated character dataset and the benchmark 3D human dataset. We provide both quantitative and qualitative analyses to support our findings.

==> writing/1_Abstract.tex <==
\begin{abstract}
Recent advances in implicit function-based approaches have shown promising results in 3D human reconstruction from a single RGB image. However, these methods often fail to generate consistent results outside the training data distribution which includes dragged or disconnected body parts, particularly in in-the-wild environments. We argue that these limitations stem from the use of existing point-level 3D shape representation which lacks in global 3D context understanding such as the relative depths among adjacent body parts. Voxel-based reconstruction methods are more suitable for capturing the entire 3D space at once and understanding holistic 3D context. However, these methods are not practical for high-resolution 3D deep learning because of their excessive memory usage. To address these challenges, we introduce Tri-directional Implicit Function (TIFu) which is a vector-level representation that increases global 3D consistencies while significantly reducing memory usage than the voxel representations. We also introduce a new method in volume construction at an arbitrary resolution by aggregating vectors along three orthogonal axes, resolving inherent problems with regressing fixed dimensions of vectors. To validate the effectiveness of our proposed method, we self-curated a challenging 3D animated character dataset available on the internet. Our approach demonstrates consistent results with in-the-wild images, significantly outperforming existing state-of-the-art methods in both our self-curated character dataset and the benchmark 3D human dataset. We provide both quantitative and qualitative analyses to support our findings.

\end{abstract}
